Unsupervised Domain-Specific Deblurring using Scale-Specific Attention

In the literature, coarse-to-fine or scale-recurrent approach i.e. progressively restoring a clean image from its low-resolution versions has been successfully employed for single image deblurring. However, a major disadvantage of existing methods is the need for paired data; i.e. sharpblur image pairs of the same scene, which is a complicated and cumbersome acquisition procedure. Additionally, due to strong supervision on loss functions, pre-trained models of such networks are strongly biased towards the blur experienced during training and tend to give sub-optimal performance when confronted by new blur kernels during inference time. To address the above issues, we propose unsupervised domain-specific deblurring using a scale-adaptive attention module (SAAM). Our network does not require supervised pairs for training, and the deblurring mechanism is primarily guided by adversarial loss, thus making our network suitable for a distribution of blur functions. Given a blurred input image, different resolutions of the same image are used in our model during training and SAAM allows for effective flow of information across the resolutions. For network training at a specific scale, SAAM attends to lower scale features as a function of the current scale. Different ablation studies show that our coarse-to-fine mechanism outperforms end-to-end unsupervised models and SAAM is able to attend better compared to attention models used in literature. Qualitative and quantitative comparisons (on no-reference metrics) show that our method outperforms prior unsupervised methods.

==> name.tex <==
\begin{figure*}[t!]
% \hskip-0.7cm
  \centering
 \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/6013_marked.jpg}
    \caption{Blurred}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/6013_marked.png}
    \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/6013_marked.jpg}
    \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/6013_marked.jpg}
    \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/6013_marked.jpg}
    \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/6013_marked_x4_SR.png}
    \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/6013_marked.png}
    \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/6013_marked.jpg}
    \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/6013_marked.jpg}
    \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/6013_marked.jpg}
    \caption{Sharp}
  \end{subfigure} \\
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/red_6013.jpg}
    % \caption{Blurred}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/red_6013.png}
    % \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/red_6013.jpg}
    % \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/red_6013.jpg}
    % \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/red_6013.jpg}
    % \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/red_6013_x4_SR.png}
    % \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/red_6013.png}
    % \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/red_6013.jpg}
    % \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/red_6013.jpg}
    % \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/red_6013.jpg}
    % \caption{Sharp}
  \end{subfigure} \\
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/green_6013.jpg}
    % \caption{Blurgreen}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/green_6013.png}
    % \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/green_6013.jpg}
    % \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/green_6013.jpg}
    % \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/green_6013.jpg}
    % \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/green_6013_x4_SR.png}
    % \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/green_6013.png}
    % \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/green_6013.jpg}
    % \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/green_6013.jpg}
    % \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/green_6013.jpg}
    % \caption{Sharp}
  \end{subfigure}\\
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/blue_6013.jpg}
    % \caption{Blurblue}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/blue_6013.png}
    % \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/blue_6013.jpg}
    % \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/blue_6013.jpg}
    % \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/blue_6013.jpg}
    % \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/blue_6013_x4_SR.png}
    % \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/blue_6013.png}
    % \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/blue_6013.jpg}
    % \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/blue_6013.jpg}
    % \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/blue_6013.jpg}
    % \caption{Sharp}
  \end{subfigure}
  \caption{Visual comparisons with start of the art results on text dataset \cite{text}.}
  \label{fig:Visual_comp_text}
\end{figure*}
\begin{figure*}[t!]
% \hskip-0.7cm
  \centering
 \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/6192_marked.jpg}
    \caption{Blurred}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/6192_marked.png}
    \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/6192_marked.jpg}
    \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/6192_marked.jpg}
    \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/6192_marked.jpg}
    \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/6192_marked_x4_SR.png}
    \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/6192_marked.png}
    \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/6192_marked.jpg}
    \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/6192_marked.jpg}
    \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/6192_marked.jpg}
    \caption{Sharp}
  \end{subfigure} \\
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/red_6192.jpg}
    % \caption{Blurred}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/red_6192.png}
    % \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/red_6192.jpg}
    % \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/red_6192.jpg}
    % \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/red_6192.jpg}
    % \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/red_6192_x4_SR.png}
    % \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/red_6192.png}
    % \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/red_6192.jpg}
    % \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/red_6192.jpg}
    % \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/red_6192.jpg}
    % \caption{Sharp}
  \end{subfigure} \\
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/green_6192.jpg}
    % \caption{Blurgreen}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/green_6192.png}
    % \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/green_6192.jpg}
    % \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/green_6192.jpg}
    % \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/green_6192.jpg}
    % \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/green_6192_x4_SR.png}
    % \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/green_6192.png}
    % \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/green_6192.jpg}
    % \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/green_6192.jpg}
    % \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/green_6192.jpg}
    % \caption{Sharp}
  \end{subfigure}\\
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/blue_6192.jpg}
    % \caption{Blurblue}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/blue_6192.png}
    % \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/blue_6192.jpg}
    % \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/blue_6192.jpg}
    % \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/blue_6192.jpg}
    % \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/blue_6192_x4_SR.png}
    % \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/blue_6192.png}
    % \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/blue_6192.jpg}
    % \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/blue_6192.jpg}
    % \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/blue_6192.jpg}
    % \caption{Sharp}
  \end{subfigure}
  \caption{Visual comparisons with start of the art results on text dataset \cite{text}.}
  \label{fig:Visual_comp_text}
\end{figure*}
\begin{figure*}[t!]
% \hskip-0.7cm
  \centering
 \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/6217_marked.jpg}
    \caption{Blurred}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/6217_marked.png}
    \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/6217_marked.jpg}
    \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/6217_marked.jpg}
    \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/6217_marked.jpg}
    \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/6217_marked_x4_SR.png}
    \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/6217_marked.png}
    \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/6217_marked.jpg}
    \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/6217_marked.jpg}
    \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/6217_marked.jpg}
    \caption{Sharp}
  \end{subfigure} \\
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/red_6217.jpg}
    % \caption{Blurred}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/red_6217.png}
    % \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/red_6217.jpg}
    % \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/red_6217.jpg}
    % \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/red_6217.jpg}
    % \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/red_6217_x4_SR.png}
    % \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/red_6217.png}
    % \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/red_6217.jpg}
    % \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/red_6217.jpg}
    % \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/red_6217.jpg}
    % \caption{Sharp}
  \end{subfigure} \\
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/green_6217.jpg}
    % \caption{Blurgreen}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/green_6217.png}
    % \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/green_6217.jpg}
    % \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/green_6217.jpg}
    % \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/green_6217.jpg}
    % \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/green_6217_x4_SR.png}
    % \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/green_6217.png}
    % \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/green_6217.jpg}
    % \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/green_6217.jpg}
    % \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/green_6217.jpg}
    % \caption{Sharp}
  \end{subfigure}\\
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Input/blue_6217.jpg}
    % \caption{Blurblue}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/NAH/blue_6217.png}
    % \caption{\cite{nah2017deep}}
  \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG1/blue_6217.jpg}
    % \caption{\cite{kupyn2018deblurgan}}
    \end{subfigure}
   \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DG2/blue_6217.jpg}
    % \caption{\cite{deblurganv2}}
    \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/DMHMP/blue_6217.jpg}
    % \caption{\cite{zhang2019deep}}
  \end{subfigure}\\
 
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/CVPR_2020/blue_6217_x4_SR.png}
    % \caption{\cite{suin2020spatially}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Cycle_GAN/blue_6217.png}
    % \caption{\cite{cyclegan}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Unsupervised/blue_6217.jpg}
    % \caption{\cite{lu2019unsupervised}}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Ours/blue_6217.jpg}
    % \caption{Ours}
  \end{subfigure}
  \begin{subfigure}[b]{0.15\linewidth}
    \includegraphics[width=\linewidth]{Supple_images/Target/blue_6217.jpg}
    % \caption{Sharp}
  \end{subfigure}
  \caption{Visual comparisons with start of the art results on text dataset \cite{text}.}
  \label{fig:Visual_comp_text}
\end{figure*}
